Extension of B-spline Material Point Method for unstructured triangular grids using Powell-Sabin splines

The Material Point Method (MPM) is a numerical technique that combines a fixed Eulerian background grid and Lagrangian point masses to simulate materials which undergo large deformations. Within the original MPM, discontinuous gradients of the piecewise-linear basis functions lead to so-called `grid-crossing errors' when particles cross element boundaries. Previous research has shown that B-spline MPM (BSMPM) is a viable alternative not only to MPM, but also to more advanced versions of the method that are designed to reduce the grid-crossing errors. In contrast to many other MPM-related methods, BSMPM has been used exclusively on structured rectangular domains, considerably limiting its range of applicability. In this paper, we present an extension of BSMPM to unstructured triangulations. The proposed approach combines MPM with $C^1$-continuous high-order Powell-Sabin (PS) spline basis functions. Numerical results demonstrate the potential of these basis functions within MPM in terms of grid-crossing-error elimination and higher-order convergence.

==> CommentedOut.tex <==

\begin{comment}
Two grids are considered for this benchmark, as shown in Figure~\ref{fig:GridSoilColumn}. For both grids, the time step size was $\Delta t\cdot 10^{-3}$ s, resulting a Courant number of approximately $C=0.2$ for both cases. The simulation remains stable and yields good results for the coarse grid, whereas the fine grid shows instabilities the moment the top triangle becomes almost empty due to the ill-conditioning of the consistent mass matrix. 

Figure~\ref{fig:SoilColumnResults} shows comparable to the results obtained with a reference UL-FEM solution from the one-dimensional analogue of the benchmark. 
This PS-MPM simulation remained stable because all main-triangles remained sufficiently filled throughout the simulation, and therefore all PS-basis functions had sufficient support such that the mass matrix $\boldsymbol{M}$ did not become ill-conditioned. 

Next, we consider the same soil column, but with grid 2, of which all triangles are half as tall as the triangles in grid 1. According to the displacement predicted by the last simulation, one of the main triangles becomes completely empty during the simulation, which can also be viewed in Figure~\ref{fig:SoilColumnGrid1}.
\end{comment}


\begin{comment}
\begin{figure}[htb]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
		\begin{center}
			\def\svgwidth{1.0\columnwidth}
			\input{images/SoilColumn2D.pdf_tex}
			\caption{Soil column benchmark}
			\label{fig:SoilColumn2D}
		\end{center}
	\end{subfigure}
	\hspace{0.03\linewidth}
	\begin{subfigure}[t]{0.35\linewidth}
		\centering
		\includegraphics[width=0.4\textwidth]{SoilcolumnGrid1.pdf}
		\includegraphics[width=0.4\textwidth]{SoilcolumnGrid1+.pdf}
		\caption{Grid 1, initially (left) and at $t=0.186$ (right).}
		\label{fig:SoilColumnGrid1}
	\end{subfigure}
	\hspace{0.03\linewidth}
	\begin{subfigure}[t]{0.35\linewidth}
		\centering
		\includegraphics[width=0.4\textwidth]{SoilcolumnGrid2.pdf}
		\includegraphics[width=0.4\textwidth]{SoilcolumnGrid2+.pdf}
		\caption{Grid 2, initially (left) and at $t=0.186$ (right).}
		\label{fig:SoilColumnGrid2}
	\end{subfigure}
	\caption{The soil column benchmark and two discretisations. A coarse discretisation is shown, as well as a discretisation which is twice as refined in the $y$-direction. Both discretisations are also shown with the expected material point positions at the largest deformation.}
	\label{fig:GridSoilColumn}
\end{figure}
\end{comment}




\begin{comment}
\begin{figure}[tbh]
	\begin{subfigure}{0.48\linewidth}
	    \centering
		\includegraphics[width=1.0\textwidth]{SoilColumnDisplacement.pdf}
		\caption{Result for grid 1, the simulation remained stable. The $y$-displacement of the middle particle over time is shown.}
		\label{fig:SimulationStable}
	\end{subfigure}
	\hspace{0.02\linewidth}
	\begin{subfigure}{0.48\linewidth}
	    \centering
		\includegraphics[width=0.4\textwidth]{SoilColumnInstable1.pdf}
		\includegraphics[width=0.4\textwidth]{SoilColumnInstable2.pdf}
		\caption{Result for grid 2, the simulation became unstable. The particle positions are shown at the step before (left) and after (right) the simulation became unstable.}
		\label{fig:SimulationUnstable}
	\end{subfigure}
    \caption{The results for the simulations with grid 1 (left) and grid 2 (right). }
	\label{fig:SoilColumnResults}
\end{figure}

The occurring instabilities for the simulation with grid 2 are not a new phenomenon within MPM~\cite{Love2006}. The acceleration field is updated as a linear combination of basis functions by solving Equation~\ref{eq:SystemOfEqs2}, $\boldsymbol{M}\boldsymbol{a}=\boldsymbol{F}$, with $M_{ij}=\sum_{p=1}^{n_p} m_p \phi_i(\boldsymbol{x}_p^t) \phi_j(\boldsymbol{x}_p^t)$.
However, as parts of the domain becomes empty or sparse, a basis function $\phi_i$ with its only support in these parts will lead to an entire row $i$ with small entries $M_{ij}$, causing an ill-conditioned mass matrix and thus resulting in instabilities when $\boldsymbol{M}\boldsymbol{a}=\boldsymbol{F}$ is solved consistently. One of the most common techniques to overcome this is by replacing the mass matrix by its lumped variant. Within this technique, a lumped mass matrix, ${\tilde{\boldsymbol{M}}}$, is created by lumping the entries of each row of $\boldsymbol{M}$ onto the diagonal. Due to the property of unity, $\sum_{k=1}^{n_p}\phi_k=1$, this becomes
\begin{equation}
    \tilde{M}_{ij} =
    \begin{cases}
        \sum_{k=1}^{n_p} M_{ik} = \sum_{p=1}^{n_p} m_p \phi_i(\boldsymbol{x}_p) \quad & \text{ if }i=j, \\
        \centering 0 \quad & \text{ if }i\neq j
    \end{cases}
\end{equation}
As the lumped mass matrix is diagonal, solving the system $\tilde{\boldsymbol{M}}\boldsymbol{a}=\boldsymbol{F}$ is equivalent to $a_i=F_i/\tilde{M}_{ii}$, which is known to greatly increase stability, even for small entries \eqref{eq:SystemVelocityProjection}. $\boldsymbol{M}^t\boldsymbol{\hat{v}}^{t+\Delta t}_k=\boldsymbol{P}^{t+\Delta t}_k$ is replaced with its lumped variant as well, resulting in a fully lumped version of PS-MPM that should remain stable, even when basis function have very little support. 
To show that this is indeed the case, the soil column benchmark has been simulated again for with the grid in Figure~\ref{fig:SoilColumnGrid2}, with the same specification as before, except that lumped PS-MPM is used instead of the consistent one. The resulting simulation remained stable, and the $y$-displacement for a particle in the middle of the column is shown in Figure~\ref{fig:ydisp_DisabledNodesLumped}. However, it can be noticed that there is a larger mismatch with the UL-FEM solution compared to the unlumped PS-MPM simulation in Figure~\ref{fig:SimulationStable}. Upon further research, we have found that the lumping has caused an oscillating stress profile, as shown in Figure~\ref{fig:yvel_DisabledNodesLumped}. Likewise, the velocity and displacement profiles throughout the soil column show similar oscillations. The oscillations are highly correlated to the grid, as shown in Figure~\ref{fig:StressProfile}. Apparently, the lumping process puts too much mass on certain basis function, extracting mass from neighbouring nodes, causing oscillations when the acceleration and velocity and solved. 
\end{comment}



For the considered soil-column benchmark, we may mitigate the oscillations caused by lumping by applying partial lumping instead of full lumping. Lumping is mostly necessary for rows in the mass matrix corresponding to basis functions with insignificant support, whereas the other basis function have sufficient support. Therefore, a stable simulation may also be ensured by only lumping the rows for the basis functions with insufficient support. A partially lumped PS-MPM variant is obtained by only lumping the rows of the basis functions which have at least one empty main-triangle in its molecule. For the considered soil column benchmark, additional empty elements are added at the top of the column, to ensure that the top most basis functions are always lumped. 


Further simulations have pointed out that larger oscillations appear as more rows of the mass matrix are lumped, whereas lumping too few rows will cause again instabilities. 


We have shown that partial lumping in PS-MPM may improve the performance of the method, but it should be mentioned that this improvement is not sufficient to be competitive with even standard lumped MPM. For an arbitrary benchmark, it may be unclear which rows to lump and which not, and stability cannot be guaranteed when using partial lumping. In many cases, it will be required to lump a significant amount of the used rows, which will cause error comparable or larger than the grid-crossing errors in standard lumped MPM. 


However, the method is still incomplete, as it suffers from severe errors when the mass matrix is lumped, whereas these error do not occur so severely in standard lumped MPM. Further research will focus on identifying the cause of this lumping error and techniques to mitigate it. Investigation of alternative unstructured spline technologies, in particular, refinable $C^1$ splines on irregular quadrilateral grids~\cite{Nguyen2016} is underway.




\begin{comment}
\begin{figure}[tbh]
	\centering
	\begin{subfigure}{0.49\linewidth}
    \centering
	\includegraphics[height=0.9\textwidth]{StressGridLumped.png}
	\label{fig:StressProfileLumped}
	\end{subfigure}
	\begin{subfigure}{0.49\linewidth}
    \centering
	\includegraphics[height=0.9\textwidth]{StressGridPartiallyLumped.png}
	\label{fig:StressProfilePartiallyLumped}
	\end{subfigure}
    \caption{The results for the simulations with a $1\times8$ block grid using fully and partially lumped PS-spline MPM.}
	\label{fig:StressProfile}
\end{figure}
\end{comment}

















\begin{appendices}
\section{Powell-Sabin spline basis functions}\label{sec:PS}
In this section, Powell-Sabin (PS) spline basis functions \cite{dierckx1992algorithms, dierckx1997calculating} are considered, which are $C^1$-continuous piece-wise quadratic splines defined on an unstructured triangulation. Furthermore, these PS-splines exhibit the partition of unity property and are non-negative over their entire support, which is local as in classical FEM. A preview of these basis functions can be found in Figure~\ref{fig:BsplineBasisFunction}. For completeness of this work, the construction process of PS-splines is summarised here shortly from the work of Dierckx \cite{dierckx1992algorithms, dierckx1997calculating}. 

\subsection{Powell-Sabin grid refinement}
To construct PS-splines, a triangulation $\Delta$ of a planar domain $\Omega$ has to be refined to a so-called Powell-Sabin refinement $\Delta^*$ \cite{powell1977piecewise}. A possible refinement $\Delta^*$ is shown in Figure~\ref{fig:PSRefinement}, which can be constructed in the following way:
\begin{enumerate}
	\item For each triangle $t_j$, choose an interior point $Z_j$, such that if two triangles $t_j$ and $t_m$ have a common edge, the line between $Z_j$ and $Z_m$ intersects the edge. The intersection point is called $Z_{jm}$. A way to guarantee the existence of the point $Z_{jm}$ is by choosing all $Z_j$ as the incenter of its triangle $t_j$. 
	\item Connect all $Z_j$ to the vertices of its triangle $t_j$ with straight lines.
	\item For each triangle $t_j$, connect the interior point $Z_j$ to all edge points $Z_{jm}$ with straight lines. In case $t_j$ is a boundary element, connect $Z_j$ to an arbitrary point on each boundary edge, for example the edge middle.
\end{enumerate}

\begin{figure}[h tb]
	\begin{center}
		\centering
		\def\svgwidth{0.5\columnwidth}
		\input{images/PSRefinement.pdf_tex}
		\caption{A PS-refinement $\Delta^*$ (solid and dashed lines) of a triangulation $\Delta$ (solid lines only). The molecule $\Omega_i$ around vertex $V_i$ is marked grey. }
		\label{fig:PSRefinement}
	\end{center}
\end{figure}
It is known that any $C^1$-continuous function, that is piece-wise quadratic on the refined triangles of $\Delta^*$, can be constructed as a linear combination of $3n_v$ Powell-Sabin basis functions, where $n_v$ is the number of vertices in the original triangulation $\Delta$ \cite{dierckx1997calculating, powell1977piecewise}. The construction procedure that three basis functions are associated with each vertex and posses the properties of non-negativity and $C^1$-continuity. Let the union of the unrefined triangles directly around $V_i$ be called the \textit{molecule} $\Omega_i$, as shown as the grey area in Figure~\ref{fig:PSRefinement}. Each basis function is locally defined around its associated vertex $V_i$ and only non-zero inside its molecule $\Omega_i$. At the molecule edge, the basis function smoothly vanishes to ensure $C^1$-continuity. To construct PS-splines that posses these properties, control triangles have to be created first around each vertex. From these control triangles, the PS-splines are then created. 

\subsection{Control Triangles}

Control triangles are created to define suitable non-negative PS-splines. For each vertex $V_i$ in the original triangulation $\Delta$, a local set of PS-points $PS_i$ is defined consisting of $V_i$ and the midpoints of all edges in the PS-refinement $\Delta^*$ with $V_i$ at one end, as shown with dots in Figure~\ref{fig:PSPoints}. To ensure non-negative basis functions, a control triangle is constructed containing all PS-points in $PS_i$. 
The control triangle is not uniquely defined, as shown in Figure~\ref{fig:PSPoints}. 
To produce PS-splines with good stability properties, the control triangle should have a small area \cite{speleers2012isogeometric}. A sufficiently good PS-triangle can be constructed by considering only control triangles with two or three edges shared with the convex hull of $PS_i$, as shown in Figure~\ref{fig:PSPoints}, and then taking the one with smallest surface. Further details about the implementation of such an algorithm can be found in \cite{koster2018towards}.

\begin{figure}[bth]
	\centering
	\begin{subfigure}[b]{0.35\textwidth}
		\begin{center}
			\def\svgwidth{0.9\columnwidth}
			\input{images/PSPoints2Edge.pdf_tex}
			%\caption{2 common edges.}
			\label{fig:PSPoints2Edge}
		\end{center}
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\begin{center}
			\def\svgwidth{0.9\columnwidth}
			\input{images/PSPoints3Edge.pdf_tex}
			%\caption{3 common edges.}
			\label{fig:PSPoints3Edge}
		\end{center}
	\end{subfigure}
	\caption{The PS-points and two possible control triangles of $V_i$ are shown in the marked molecule $\Omega_i$ from the example triangulation $\Delta^*$ used earlier. The two control triangles are constructed by taking respectively two (left) and three edges (right) in common with the convex hull of $PS_i$.}
	\label{fig:PSPoints}
\end{figure}

Each control triangle defines three basis functions, all associated with vertex $V_i$ and the molecule $\Omega_i$. Therefore, the basis functions are indexed $\phi_i^q$ ($i=1,\dots, n_v,\, q=1,2,3$), where $i$ indicates the vertex $V_i$ and $q$ the local index. Each basis function $\phi_i^q$ is uniquely defined by a triplet $(\alpha_i^q, \beta_i^q, \gamma_i^q)$, containing the value and gradient of $\phi_i^q$ in its associated vertex $V_i$,
\begin{equation}\label{eq:triplet}
	\left(\alpha_{i}^q,\beta_{i}^q,\gamma_{i}^q\right)=\left(\phi_i^q(V_i),\pder{\phi_i^q}{x}(V_i),\pder{\phi_i^q}{y}(V_i)\right).
\end{equation}
The triplets of the three PS-spline basis functions corresponding to vertex $V_i$ are determined from the control triangle and the position of $V_i$. Let the Cartesian coordinates of the control triangle vertices be $Q_i^1=(X_i^1,Y_i^1)$, $Q_i^2=(X_i^2,Y_i^2)$ and $Q_i^3=(X_i^3,Y_i^3)$, and the Cartesian coordinates of $V_i= (x_i,y_i)$. The three triplets are then determined by solving
\begin{align}
	\begin{bmatrix}
	X^1_i & X^2_i & X^3_i\\
	Y^1_i & Y^2_i & Y^3_i\\
	1 & 1 & 1
	\end{bmatrix}
	\begin{bmatrix}
	\alpha^1_i & \beta^1_i & \gamma^1_i\\
	\alpha^2_i & \beta^2_i & \gamma^2_i\\
	\alpha^3_i & \beta^3_i & \gamma^3_i
	\end{bmatrix}
	=&
	\begin{bmatrix}
	x_i & 1 & 0\\
	y_i & 0 & 1\\
	1   & 0 & 0
	\end{bmatrix}. \label{eq:AlphaBetaGamma}
\end{align}

The control triangle has a direct geometric interpretation for the triplet. Solving for the triplet $\left(\alpha_{i}^q,\beta_{i}^q,\gamma_{i}^q\right)$ of a basis function $\phi_i^q$ corresponds geometrically to `lifting' up control triangle vertex $Q_i^q$ of the control triangle in the $z$-direction and evaluating the height and gradient of the resulting plane at the location of $V_i$, see Figure~\ref{fig:LiftedPlane}.

\begin{figure}[htb]
    \centering
	\includegraphics[width=1\textwidth]{images/PS-pointsLifted.pdf}
	\caption{A control triangle lifted to $z=1$ in one of its vertices for determining a triplet of a basis function. The location in the lifted plane above the vertex $V_i$ in the middle is marked with a dot; the value and gradient there correspond to the triplet of the associated basis function.}
	\label{fig:LiftedPlane}
\end{figure}


\subsection{Bernstein-B\'ezier formulation for quadratic splines}

From the triplet $\left(\alpha_{i}^q,\beta_{i}^q,\gamma_{i}^q\right)$, the PS-spline $\phi_i^q$ can be constructed as a piece-wise quadratic polynomial over each sub-triangle in $\Delta^*$ using barycentric coordinates. Cartesian coordinates $(x,y)$ can be converted to barycentric coordinates $(\eta_1,\eta_2,\eta_3)$ with respect to the considered triangle vertices $(x_1,y_1),(x_2,y_2),(x_3,y_3)$ as follows,
\begin{equation}\label{eq:BarycentricCoordinates}
	\begin{bmatrix}
	x_1 & x_2 & x_3 \\
	y_1 & y_2 & y_3 \\
	1 & 1 & 1 
	\end{bmatrix}
	\begin{bmatrix}
	\eta_1 \\
	\eta_2 \\
	\eta_3  
	\end{bmatrix}
	=
	\begin{bmatrix}
	x \\
	y \\
	1  
	\end{bmatrix}.
\end{equation}
In Figure~\ref{fig:BezierOrdinatesTriangle}, some barycentric coordinates are shown with respect to the shown triangle.

To construct a single basis function over each sub-triangle $st$, $6$ quadratic Bernstein polynomials $B_{i,j,k}$ are defined in barycentric coordinates,
\begin{equation}\label{eq:BernsteinPolynomial}
	B_{i,j,k}(\boldsymbol{\eta}) = \frac{2!}{i!j!k!}\eta_1^i\eta_2^j\eta_3^k,\quad\text{with } i,j,k\in\{0,1,2\},\quad\text{and}\quad i+j+k=2,
\end{equation}
which are non-negative and form a partition of unity.
%\begin{align*}
%    B_{i,j,k}(\boldsymbol{\eta}) &\geq 0, \quad \, \forall (x,y)\in st,\\
%	\sum_{\substack{i+j+k=2,\\ i,j,k\geq 0}}B_{i,j,k}(\boldsymbol{\eta}) &= 0, \quad \forall \, (x,y)\in st.
%\end{align*}
Any desired quadratic polynomial $b(\boldsymbol{\eta})$ can be uniquely constructed as a linear combination of the $6$ quadratic Bernstein polynomials $B_{i,j,k}$ over a sub-triangle $st$,
\begin{equation}\label{eq:BernsteinBezier}
	b(\boldsymbol{\eta})=\sum_{\substack{i+j+k=2,\\ i,j,k\in\{0,1,2\}}}b_{i,j,k}B_{i,j,k}(\boldsymbol{\eta}),
\end{equation}
where $b_{i,j,k}$ are called the B\'ezier ordinates. 
The desired quadratic polynomial can thus be fully defined by its B\'ezier ordinates, which can be schematically represented by associating B\'ezier ordinate $b_{i,j,k}$ with barycentric coordinates $\left(\tfrac{i}{2},\tfrac{j}{2},\tfrac{k}{2}\right)$, as shown in Figure~\ref{fig:BezierOrdinatesTriangle}.
\begin{figure}[tbh]
\begin{center}
    \begin{subfigure}[b]{0.45\textwidth}
	    \centering
		\def\svgwidth{1\columnwidth}
		\input{images/2DRefinement.pdf_tex}
		%\caption{}
	%	\caption{Barycentric coordinates of a triangle with respect to its vertices.}
	    \centering{Barycentric coordinates}
		\label{fig:BarycentricCoordinates}
	\end{subfigure}
	\hspace{0.3cm}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\def\svgwidth{1\columnwidth}
		\input{images/BezierOrdinatesTriangle.pdf_tex}
	    \centering{B\'ezier ordinates}
	    %\caption{}
	%	\caption{B\'ezier ordinates at the corresponding barycentric coordinates.}
	\end{subfigure}
\end{center}
	\caption{Barycentric coordinates with respect to the sub-triangle vertices (left) and the B\'ezier ordinates of  a quadratic polynomial $b(\boldsymbol{\eta})$ (right), schematically represented at the same location.}
    \label{fig:BezierOrdinatesTriangle}
\end{figure}	

\subsection{Construction of PS-splines}
Next, consider the molecule $\Omega_i$ around a vertex $V_i$ and one of the main-triangles $t_j$ in the molecule, as depicted in Figure~\ref{fig:BezierOrdinatesSubTriangles}. The grey main-triangle has been divided into 6 sub-triangles in the refinement $\Delta^*$. In each of the sub-triangles, the $6$ locations with barycentric coordinates $\left(\tfrac{i}{2},\tfrac{j}{2},\tfrac{k}{2}\right),\,i+j+k=2,\, i,j,k\in\{0,1,2\}$ have been marked.
Denote the vertices of the main-triangle by $v_1$, $v_2$ and $v_3$, with $v_1$ $(=V_i)$ the middle vertex of the considered molecule, and let $v_2$ and $v_3$ be indexed counter-clockwise. Let the center vertex $Z$ of the grey triangle have barycentric coordinates $Z=(a,b,c)$ with respect to vertices $v_1$, $v_2$ and $v_3$.
Furthermore, let the edge vertices $R$ have barycentric coordinates $R_{12}=(\lambda_1,\lambda_2,0)$, $R_{23}=(0,\mu_2,\mu_3)$ and $R_{13}=(\nu_1,0,\nu_3)$, as denoted in Figure~\ref{fig:BezierOrdinatesSubTriangles}. 
Finally, let $v_1$ have barycentric coordinates $v_1=(\alpha_i^1,\alpha_i^2,\alpha_i^3)$ with respect to the control triangle vertices $Q_i^1$, $Q_i^2$ and $Q_i^3$.
These values of $\alpha$ also correspond to the first values of the three triplets of the basis functions associated with this molecule, see Equation~\ref{eq:AlphaBetaGamma}. 
\begin{figure}[tbh]
	\begin{center}
		\centering
		\def\svgwidth{\columnwidth}
		\input{images/BezierOrdinatesSubTriangles.pdf_tex}
		\caption{Left: the molecule around a vertex $V_i$. Right: one of the main-triangles in the molecule. The locations of the middle vertex $Z$ and the edge vertices $R$ are marked with respect to the vertices $v_1$, $v_2$ and $v_3$. $v_1(=V_i)$ is also marked with the barycentric coordinates with respect to the control triangle. }
		\label{fig:BezierOrdinatesSubTriangles}
	\end{center}
\end{figure}

Finally, the three basis function $\phi_i^q,\, q=1,2,3$, associated with vertex $V_i$ are defined by their B\'ezier ordinates on each of the triangles in the molecule around $V_i$. The B\'ezier ordinates of a basis function $\phi_i^q$ are shown in Figure~\ref{fig:BezierOrdinates}. The coefficients in the figure are given in terms of the triplet $(\alpha,\beta,\gamma)=(\alpha_i^q,\beta_i^q,\gamma_i^q)$ of the considered basis function $\phi_i^q$ and the barycentric coordinates of $Z=(a,b,c)$, $R_{12}=(\lambda_1,\lambda_2,0)$, $R_{13}=(\nu_1,0,\nu_3)$, and the Cartesian coordinates of the considered triangle $v_1=(x_1,y_1)$, $v_2=(x_2,y_2)$ and $v_3=(x_3,y_3)$ as follows,
\begin{align}
	L=\,\alpha+\frac{1-\lambda_1}{2}\overline{\beta}, \qquad
	L'=\,\alpha+\frac{1-\nu_1}{2}\overline{\gamma}, \qquad
	\tilde{L}=\,\alpha+\frac{b}{2}\overline{\beta}+\frac{c}{2}\overline{\gamma},
	\end{align}
	with
	\begin{align}
	\overline{\beta}=\beta(x_2-x_1)+\gamma(y_2-y_1) \quad \text{and} \quad
	\overline{\gamma}=\beta(x_3-x_1)+\gamma(y_3-y_1).
\end{align}
\begin{figure}[h!tb]
\begin{center}
	\centering
	\def\svgwidth{0.45\columnwidth}
	\input{images/BezierOrdinates.pdf_tex}
	\caption{The B\'ezier ordinates for basis function $\phi_i^1$, corresponding to the vertex $V_i$ considered in Figure~\ref{fig:BezierOrdinatesSubTriangles}. There are three different basis functions, note that for each of these basis functions, $\alpha$, $\beta$ and $\gamma$ should correspond with the triplet $(\alpha^q,\beta^q,\gamma^q)$ corresponding to PS-triangle vertex $Q_q$.}
	\label{fig:BezierOrdinates}
\end{center}
\end{figure}
The three resulting PS-splines corresponding to the shown control triangle of vertex $V_i$ are shown on the associated molecule $\Omega_i$ in Figure~\ref{fig:BsplineBasisFunction}. 
\begin{figure}[htb]
	\begin{subfigure}[b]{0.45\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{images/PS-splinePlot3.png}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{images/PS-splinePlot2.png}
	\end{subfigure}
	\center{
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
	    \includegraphics[width=\textwidth]{images/PS-splinePlot1.png}
	\end{subfigure}}
	\caption{The three $C^1$-continuous PS-spline basis function corresponding to the middle vertex, constructed from the marked control triangle.}
    \label{fig:BsplineBasisFunction}
\end{figure}

\subsection{PS-splines in MPM}
Throughout this paper, the resulting PS-splines are adopted as basis functions within MPM. Since each vertex is associated with three basis functions, PS-spline MPM uses three times as many basis functions compared to standard MPM for the same grid. However, the spatial function reconstruction of PS-splines is known to be of third order for smooth functions, in contrast to the second-order spatial convergence of piece-wise linear basis functions \cite{speleers2012isogeometric, koster2018towards}, so a coarser grid can be used in case of PS-splines for a comparable precision. 

The basis functions can be stored per main triangle, each with nine non-zero basis functions: three basis functions $\phi_i^q$, $q=1,2,3$ for each of its three vertices $V_i$. Each of these basis functions is fully defined on this main triangle by its nine non-zero B\'ezier ordinates as depicted in Figure~\ref{fig:BezierOrdinates}. The value of a basis function in a certain location $\boldsymbol{x}^*$ can then be retrieved by first finding the sub-triangle in which $\boldsymbol{x}^*$ is located, then finding its barycentric coordinates $(\eta_1,\eta_2,\eta_3)$ with respect to that sub-triangle, and finally applying the Bernstein-B\'ezier formulation from Equations~\ref{eq:BernsteinPolynomial} and \ref{eq:BernsteinBezier}. 

At the location of each boundary vertex $V_i$, at most three basis functions are non-zero, each of which has a known triplet describing the value and gradient at the vertex. A Dirichlet boundary condition, arising in the benchmark considered in this paper, can be applied by imposing that the the value of the reconstructed field in $V_i$ is equal to the imposed value,
\begin{equation}
    f(V_i) = \sum_{j=1}^{n_v}\sum_{q=1}^3c_j^q \phi_j^q(V_i) = \sum_{q=1}^3c_i^q \phi_i^q(V_i) = \sum_{q=1}^3c_i^q \alpha_i^q. 
\end{equation}
The Dirichlet condition can also be implemented by imposing that the partial derivative tangent to the boundary in $V_i$ is equal for the boundary condition and the reconstructed field,
\begin{equation}
    \nabla f(V_i)\cdot \boldsymbol{\hat{r}}(V_i) =
    \sum_{q=1}^3 c_i^q \nabla\phi_i^q \cdot \boldsymbol{\hat{r}} = 
    \sum_{q=1}^3 c_i^q (\beta_i^q \hat{r}_x + \gamma_i^q\hat{r}_y),
\end{equation}
where $\boldsymbol{\hat{r}}$ is the tangent to the boundary.


\end{appendices}

